An existence proof for the gravitating BPS monopole

We prove the existence of the gravitating BPS monopole in Einstein-Yang-Mills-Higgs (EYMH) theory. Existence is established using a Newtonian perturbation argument which shows that a Yang-Mills-Higgs BPS monopole solution can be be continued analytically in powers of $1/c^{2}$ to an EYMH solution.

==> limit.tex <==
\sect{limit}{The formal limit $\lambda \rightarrow 0$}


We assume that all the  fields are static and that $\partial_{0}$
is a timelike hypersurface orthogonal killing vector field for the
metric. Therefore
\eqn{static1}{
\partial_{0} \U^{\alpha \beta} = 0\, , \; \partial_{0} A_{\alpha} = 0\, ,\;
 \partial_{0} \Phi = 0\,
\quad \text{and}\quad \U^{j 0} = \U^{0 j} = 0\, .
}
Since $\U^{\alpha \beta}$ is symmetric, i.e $\U^{\alpha \beta} =
\U^{\beta \alpha}$, we define the following subspace of
the 4 by 4 matrices
\eqn{static3}{
\Sbb := \{\, X=(X^{\alpha \beta}) \in \Mbb_{4\times 4} \,|\, X^{\alpha \beta}
= X^{\beta \alpha} \;\text{and}\; X^{0 j} = 0 \,\}\;.
}
Then letting $\U = (\U^{\alpha\beta})$, $\U$ takes values
in $\Sbb$. We will also assume that
\eqn{static4}{
A_{0} = 0  \, .
}
Therefore
if we write the gauge potential $A_{i}$ as a 3-tuple
$A = (A_{1},A_{2},A_{3})$ then the gauge potential
$A$ takes values in the space $\sU{2}^{3}$ which
carries a norm
\eqn{gpotnorm}{
\enorm{A}^{2} := \sum_{i=1}^{3} \ip{A_{i}}{A_{i}} \, .
}
Finally, we note that the Higgs field $\Phi$ takes values in 
$\sU{2}$. 


The main virture of the field equations \eqref{reduced3} and  \eqref{YMH1}-\eqref{YMH2},
is that they are analytic in the variables 
$(\lambda,\U,\U_{,\alpha},\U_{,\alpha\beta}, A,A_{,\alpha},A_{,\alpha,\beta},\Phi,
\Phi_{,\beta},\Phi_{\alpha,\beta})$ for 
$(\lambda,\U)$ for $|\lambda|$ and $|U|$ small enought.
For the purpose of taking the formal limit, we are now treating the variables 
$\U$, $A$, $\Phi$ and there first and second derivatives as indepedent 
finite dimensional vectors and no-longer as fields on space-time.

To establish the analyticity we first note
that
\leqn{gflatupA}{
(\underset{o}{\gb}{}^{\alpha\beta}) = 
\diag(-\lambda, 1, 1, 1) \quad \text{and}
\quad (\underset{o}{\gb}{}_{\alpha\beta}) =
\diag(-1, \lambda,\lambda,\lambda)
}
so that
\leqn{gflatupB}{
(\underset{o}{\gb}{}^{\alpha\beta})\big|_{\lambda=0} = 
\diag(0,1,1,1)
\quad \text{and}
\quad (\underset{o}{\gb}{}_{\alpha\beta})\big|_{\lambda=0} =
\diag(-1,0,0,0).
}
From this and the fact that matrix inversion is analytic in a neighborhood of
the identity and the functions $(1+x)^{q/2}$ ($q=2,1,-1$) are analytic in
a neighborhood of $x=0$, it is not difficult to show that $\gb_{\alpha\beta}$ and
$\df^{q/2}$ ($q=2,1,-1$) are analytic in $(\lambda,\U)$
for  $|\lambda|$ and $|U|$ small enough and that
the following expansions are valid
\gath{HeilA2}{
\df-1 = -4\lambda \U^{00} + \Ord(\lambda^{2}) \, ,\quad
\sqrt{\df}-1 = -2\lambda \U^{00} + \Ord(\lambda^{2}) \, ,\\
\frac{1}{\sqrt{\df}}-1 = 2\lambda \U^{00} + \Ord(\lambda^{2}) \, , \quad
(\gb_{\alpha\beta} - \underset{o}{\gb}{}_{\alpha\beta}) = -4\lambda
(\delta^{0}_{\alpha}\delta^{0}_{\beta})\U^{00} + \Ord(\lambda^{2}) \, .
}
For detalis see \cite{Heil95}.  With these expansions 
it is easy to see that the Christoffel symbols \eqref{Christ} are also
analytic in $(\lambda,\U,\U_{\alpha})$ and 
\eqn{HeilB2}{
\Gamma^{\alpha}_{\beta\gamma} = \Gamma^{\alpha}_{\beta\gamma}\big|_{\lambda = 0}
+ \Ord(\lambda)
}
where
\eqn{HeilB3}{
\Gamma^{\alpha}_{\beta\gamma}\big|_{\lambda = 0} = \left\{
\begin{array}{ll} \U^{00}{}_{,\alpha} & \text{if $\beta=\gamma=0$ and
$\alpha \neq 0$}\\
0 & \text{otherwise}
\end{array} \right. \, .
} 
These expansions allow us to conclude that for $|\lambda|$ and $|\U|$
small enough 



